3D-SceneDreamer: Text-Driven 3D-Consistent Scene Generation

Text-driven 3D scene generation techniques have made rapid progress in recent years. Their success is mainly attributed to using existing generative models to iteratively perform image warping and inpainting to generate 3D scenes. However, these methods heavily rely on the outputs of existing models, leading to error accumulation in geometry and appearance that prevent the models from being used in various scenarios (e.g., outdoor and unreal scenarios). To address this limitation, we generatively refine the newly generated local views by querying and aggregating global 3D information, and then progressively generate the 3D scene. Specifically, we employ a tri-plane features-based NeRF as a unified representation of the 3D scene to constrain global 3D consistency, and propose a generative refinement network to synthesize new contents with higher quality by exploiting the natural image prior from 2D diffusion model as well as the global 3D information of the current scene. Our extensive experiments demonstrate that, in comparison to previous methods, our approach supports wide variety of scene generation and arbitrary camera trajectories with improved visual quality and 3D consistency.

==> figure/long_figure_result.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1.0\textwidth]{figure/media_supp/long_figure_result.pdf}
    % \vspace{-6mm}
    \caption{\textbf{Quantitative Results.} From our results, it can be seen that our approach produces high-fidelity scenes with stable 3D consistency in indoor scenes, outdoor scenes, and unreal-style scenes. More high-resolution results can be found in the supplementary material.}
    % \vspace{-4mm}
    \label{fig:result_supp}
\end{figure*}

==> figure/strech.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\textwidth]{figure/media/strech.pdf}
    \caption{\textbf{Observations on the generation of large-scale scenes.} The outdoor scene can lead to accumulating errors due to the limitation of mesh representation and the lack of a reasonable correction mechanism, which can be observed from the yellow box. However, our approach can alleviate the problem by introducing a novel pipeline.}
    \label{fig:strech}
    \vspace{-4mm}
\end{figure}

==> table/ablation_feature.tex <==
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cccc}
\toprule
\textbf{Inputs} &
  \cellcolor[HTML]{FEF1F1}\textbf{DE} &
  \cellcolor[HTML]{FEF1F1}\textbf{CE} &
  \cellcolor[HTML]{F0FBEF}\textbf{SfM rate} &
  \cellcolor[HTML]{F0FBEF}\textbf{CS} \\ \midrule
Course Image     & 0.71          & 1.618          & 0.61          & 23.41          \\
+depth map       & 0.68          & 0.646          & 0.42          & 28.18          \\
+depth feature   & 0.49          & 0.495          & 0.50          & 23.97          \\
+feature adapter & \textbf{0.19} & \textbf{0.198} & \textbf{0.86} & \textbf{28.71} \\ \bottomrule
\end{tabular}%
}
\vspace{-3mm}
\caption{Ablation on the conditional input of the refine model.}
\vspace{-2mm}
\label{tab:ablation_feature}
\end{table}

==> table/ablation_pose.tex <==
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
Pose Num &
  \cellcolor[HTML]{FEF1F1}\textbf{DE} &
  \cellcolor[HTML]{FEF1F1}\textbf{CE} &
  \cellcolor[HTML]{F0FBEF}\textbf{SfM rate} &
  \cellcolor[HTML]{F0FBEF}\textbf{CLIP Score} \\ \midrule
N=0  & 0.49          & 0.891          & 0.41          & 23.12          \\
N=2  & 0.28          & 0.632          & 0.49          & 25.18          \\
N=4  & 0.23          & 0.485          & 0.56          & 25.97          \\
N=8  & \textbf{0.14} & \textbf{0.179} & \textbf{0.86} & \textbf{28.71} \\
N=12 & 0.19          & 0.253          & 0.61          & 29.12          \\ \bottomrule
\end{tabular}%
}
\vspace{-3mm}
\caption{Ablation on the initial number of viewpoints.}
\vspace{-2mm}
\label{tab:ablation_pose_num}
\end{table}

==> table/compare_to_object.tex <==
\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cccc}
\toprule
\textbf{Method} &
  \cellcolor[HTML]{F0FBEF}\textbf{CS$\uparrow$} &
  \cellcolor[HTML]{FEF1F1}\textbf{BRISQUE$\downarrow$} &
  \cellcolor[HTML]{FEF1F1}\textbf{NIQE$\downarrow$} &
  \cellcolor[HTML]{F0FBEF}\textbf{IS$\uparrow$} \\ \midrule
CLIP-Mesh~\cite{CLIP_Mesh}       & 27.16          & 49.26          & 6.15          & 1.09          \\
DreamFusion~\cite{dreamfusion}     & 23.15          & 31.54          & 9.47          & 1.12          \\
ProlificDreamer~\cite{Prolificdreamer} & 21.58          & 62.02          & 8.02          & 1.20          \\
\rowcolor[HTML]{EFEFEF} 
Ours            & \textbf{28.12} & \textbf{24.15} & \textbf{4.96} & \textbf{2.62} \\ \bottomrule
\end{tabular}
}
\vspace{-3mm}
\caption{\textbf{Comparision with text-to-object methods.} We compare our method with recent text-driven 3D generation methods~\cite{dreamfusion, Prolificdreamer, CLIP_Mesh}. Metrics on visual quality are illustrated.}
\label{tab:compare_to_object}
\vspace{-2mm}
\end{table}
